Two-Loop Leading Color Corrections to Heavy-Quark Pair Production in the Gluon Fusion Channel

We evaluate the two-loop QCD diagrams contributing to the leading color coefficient of the heavy-quark pair production cross section in the gluon fusion channel. We obtain an analytic expression, which is valid for any value of the Mandelstam invariants s and t and of the heavy-quark mass m. Our findings agree with previous analytic results in the small-mass limit and with recent results for the coefficients of the IR poles.

==> numerics/Makefile <==
CPPC=g++
CFLAGS=-c -Wall
LDFLAGS=-lginac

HSOURCES=\
  ggtt_a_exact_m4_01.cpp\
  ggtt_a_exact_m3_01.cpp\
  ggtt_a_exact_m2_01.cpp\
  ggtt_a_exact_m1_01.cpp\
  ggtt_a_exact_m1_02.cpp\
  ggtt_a_exact_m1_03.cpp\
  ggtt_a_exact_0_01.cpp\
  ggtt_a_exact_0_02.cpp\
  ggtt_a_exact_0_03.cpp\
  ggtt_a_exact_0_04.cpp\
  ggtt_a_exact_0_05.cpp\
  ggtt_a_exact_0_06.cpp\
  ggtt_a_exact_0_07.cpp\
  ggtt_a_exact_0_08.cpp\
  ggtt_a_exact_0_09.cpp\
  ggtt_a_exact_0_10.cpp\
  ggtt_a_exact_0_11.cpp\
  ggtt_a_exact_0_12.cpp\
  ggtt_a_exact_0_13.cpp\
  ggtt_a_exact_0_14.cpp\
  ggtt_a_exact_0_15.cpp\
  ggtt_a_exact_0_16.cpp\
  ggtt_a_exact_0_17.cpp\
  ggtt_a_exact_0_18.cpp\
  ggtt_a_exact_0_19.cpp\
  ggtt_a_exact_0_20.cpp\
  ggtt_a_exact_0_21.cpp\
  ggtt_a_exact_0_22.cpp\
  ggtt_a_exact_0_23.cpp\
  ggtt_a_exact_0_24.cpp\
  ggtt_a_exact_0_25.cpp\
  ggtt_a_exact_0_26.cpp

HOBJECTS=$(HSOURCES:.cpp=.o)


ggtt_a: main.o ggtt_a_exact.o ggtt_a_smallbeta.o ggtt_a_smallmass.o $(HOBJECTS)
	$(CPPC) -o $@ $+ $(LDFLAGS)

ggtt_a_exact.o: ggtt_a_exact.h

ggtt_a_smallbeta.o: ggtt_a_smallbeta.h

ggtt_a_smallmass.o: ggtt_a_smallmass.h

main.o: ggtt_a_exact.h ggtt_a_smallbeta.h ggtt_a_smallmass.h

%.o: %.cpp
	$(CPPC) $(CFLAGS) $< -o $@

clean:
	rm -f *.o *~


